Census of R Coronae Borealis stars I: Infrared light curves from Palomar Gattini IR

We are undertaking the first systematic infrared (IR) census of R Coronae Borealis (RCB) stars in the Milky Way, beginning with IR light curves from the Palomar Gattini IR (PGIR) survey. PGIR is a 30 cm $J$-band telescope with a 25 deg$^{2}$ camera that is surveying 18000 deg$^{2}$ of the northern sky ($\delta>-28^{o}$) at a cadence of 2 days. We present PGIR light curves for 922 RCB candidates selected from a mid-IR color-based catalog (Tisserand et al. 2020). Of these 922, 149 are promising RCB candidates as they show pulsations or declines similar to RCB stars. Majority of the candidates that are not RCB stars are either long period variables (LPVs) or RV-Tauri stars. We identify IR color-based criteria to better distinguish between RCB stars and LPVs. As part of a pilot spectroscopic run, we obtained NIR spectra for 26 out of the 149 promising candidates and spectroscopically confirm 11 new RCB stars. We detect strong He I $\lambda 10830$ features in spectra of all RCB stars, likely originating within high velocity (200-400 km-s$^{-1}$) winds in their atmospheres. 9 of these RCB stars show $^{12}$C$^{16}$O and $^{12}$C$^{18}$O molecular absorption features, suggesting that they are formed through a white dwarf merger. We detect quasi-periodic pulsations in the light curves of 5 RCB stars. The periods range between 30-125 days and likely originate from the strange-mode instability in these stars. Our pilot run results motivate a dedicated IR spectroscopic campaign to classify all RCB candidates.

==> authors.tex <==
\author[Karambelkar et al.]{
\parbox{17.5cm}{
  V.~Karambelkar$^{1}$ \thanks{E-mail: viraj@astro.caltech.edu}, 
  %ORCID Nadia [0000-0003-0901-1606]
  M.~M.~Kasliwal$^{1}$,
  P.~Tisserand$^{2}$,
  K.~De$^{1}$,
  S. ~Anand $^{1}$,
  M.~C.~B.~Ashley$^{3}$,
  A. Delacroix$^{4}$,
  M.~Hankins$^{5}$,
  J.~E. Jencson$^{6}$,
  R.~M.~Lau$^{7}$,
  D.~McKenna$^{4}$,
  A.~Moore $^{8}$,
  E.~O.~Ofek$^{9}$,
  R.~Smith$^{4}$,
  R.~Soria$^{10,11}$,
  J.~Soon$^{8}$,
  S. Tinyanont $^{12}$,
  T.~Travouillon$^{8}$,
  Y. ~Yao $^{1}$
\\
  }
  \\
  \\
  $^{1}$ Cahill Center for Astrophysics, California Institute of Technology, Pasadena, CA 91125, USA\\
  $^{2}$ Sorbonne Universites, UPMC Univ. Paris 6 et CNRS, UMR 7095, Institut d’Astrophysique de Paris, IAP, 75014 Paris, France\\
  $^{3}$ School of Physics, University of New South Wales, Sydney, NSW 2052, Australia \\
  $^{4}$ Caltech Optical Observatories, California Institute of Technology, Pasadena, CA 91125, USA\\
  $^{5}$ Arkansas Tech University, 203 W O St, Russellville, AR 72801\\
  $^{6}$ University of Arizona, Steward Observatory, 933 N. Cherry Avenue, Tucson, AZ 85721, USA\\
  $^{7}$ Institute of Space and Astronautical Science, Japan Aerospace Exploration Agency, 3-1-1 Yoshinodai, Chuo-ku, Sagamihara,\\ Kanagawa 252-5210, Japan\\
  $^{8}$ Research School of Astronomy and Astrophysics, Australian National University, Canberra, ACT 2611, Australia\\
  $^{9}$ Department of Particle Physics and Astrophysics, Weizmann Institute of Science, Rehovot 76100, Israel\\
  $^{10}$ College of Astronomy and Space Sciences, University of the Chinese Academy of Sciences, Beijing 100049, China\\
  $^{11}$ Sydney Institute for Astronomy, School of Physics A28, The University of Sydney, Sydney, NSW 2006, Australia\\
  $^{12}$ University of California Santa Cruz, 1156 High St, Santa Cruz, CA 95064\\
}


==> known_rcbs.tex <==
\begingroup
\renewcommand{\tabcolsep}{2pt}
\begin{table*}
\begin{center}
\begin{minipage}{16cm}
\caption{Catalog of RCBs}
\label{tab:candidate_list}
\begin{tabular}{ccccccc}
\hline
\hline
{Candidate} & {R.A} & {Dec} & {Photometric} & {Spectroscopic} & {Mean J} & {Observation} \\ 
{I.D} & {(deg)} & {(deg)} & {Class} & {Class} & (mag) & {Date}\\
\hline
2 &  &  &  Fading  &     &    \\
6 &  &  &  Fading &  RCB &      \\
\hline
\hline
\end{tabular}
\begin{tablenotes} \item References: \end{tablenotes}
\end{minipage}
\end{center}
\end{table*}
\endgroup

==> table_colpris.tex <==
\begingroup
\renewcommand{\tabcolsep}{2pt}
\begin{table*}
\begin{center}
\begin{minipage}{16cm}
\caption{IR color based priorities for the 2194 candidates in \citet{Tisserand2020}.}
\label{tab:colpris}
\begin{tabular}{cccc}
\hline
\hline
{WISE} & {R.A} & {Dec} & {Color-based} \\ 
{ToI} & {(deg)} & {(deg)} & {Priority} \\
\hline
1 & 2.1755 & 63.0093 & 1-b\\
2 & 4.7942 & 52.0343 & 1-a\\
... & & & \\
\hline
\hline
\end{tabular}
\begin{tablenotes}
 \item This table is published online in its entirety in the machine-readable format.
\end{tablenotes}
\end{minipage}
\end{center}
\end{table*}
\endgroup

==> table_spec_anal_old.tex <==
\begingroup
\renewcommand{\tabcolsep}{2pt}
\begin{table*}
\begin{minipage}{8cm}
\caption{Properties derived from the spectra of RCB stars}
\label{tab:helium}
\begin{tabular}{cccccc}
\hline
\hline
{RCB} & RV $^{a}$ & {$T_{\mathrm{eff}}^{b}$} & O$^{16}$/O$^{18}$ $^{c}$ & {EW$^{d}$} & {v$_{m}^{e}$} \\ 
{Name} & {km/s} & K & & {A} & {km-s$^{-1}$}  \\
\hline
AO Her & 500 & 5250 & 10 & 13.9 & 500 \\
NSV11154 & 300 & 5750 & 10 & 4.9 & 325 \\
WISE J17+ & 0 & 5500 & 2 & 2.3 & 300 \\
ASAS-RCB-21 & -50 & 6000 & 2  & 2.2 & 350 \\
V391 Sct & 0 & & & 4.8 & 300 \\
WISE J18+ & -150 & 6000 & 1 & 1.7 & 330 \\
WISE-ToI-6 & 0 & & & 6.0 & 450\\
%WISE-RCB-8 &  & \\
WISE-ToI-223 & -100 & 6000 & 2 & 12.0 & 550\\
WISE-ToI-268 & -150 & 5750 & 10 & 10.6 & 400 \\
WISE-ToI-274 & 0 & 5750 & 5 & 8.6 & 330\\
WISE-ToI-281 & 0 & 6250 & 5 & 8.5 & 300\\
WISE-ToI-1309 & 0 & & & 11.6 & 500\\
\hline
\hline
\end{tabular}
\begin{tablenotes} 
\item $a$ : Radial velocity of the RCB star. We estimate an uncertainty of 50 km/s on the measurements. 
\item $b$ : Photospheric temperature of the RCB star. The uncertainty on the value is 250 K.
\item $c$ : Oxygen isotope ratios. The values are uncertain by a factor of two.
\item $d$ : Equivalent width of the Helium absorption profile. 
\item $e$ : Maximum velocity of the Helium absorption profile.
\end{tablenotes}
\end{minipage}
\end{table*}
\endgroup

==> table_spec_anal_old_v2.tex <==
\begingroup
\renewcommand{\tabcolsep}{2pt}
\begin{table*}
\begin{minipage}{8cm}
\caption{Properties derived from the spectra of RCB stars}
\label{tab:helium}
\begin{tabular}{cccc}
\hline
\hline
{RCB} & RV $^{a}$ & {$T_{\mathrm{eff}}^{b}$} & O$^{16}$/O$^{18}$ $^{c}$ \\ 
{Name} & {km-s$^{-1}$} & K & \\
\hline
AO Her & 500 & 5250 & 10  \\
NSV11154 & 300 & 5750 & 10 \\
WISE J17+ & 0 & 5500 & 2  \\
ASAS-RCB-21 & -50 & 6000 & 2  \\
V391 Sct & 0 & & \\
WISE J18+ & -150 & 6000 & 1  \\
WISE-ToI-6 & 0 & & \\
%WISE-RCB-8 &  & \\
WISE-ToI-223 & -100 & 6000 & 2 \\
WISE-ToI-268 & -150 & 5750 & 10 \\
WISE-ToI-274 & 0 & 5750 & 5 \\
WISE-ToI-281 & 0 & 6250 & 5 \\
WISE-ToI-1309 & 0 & & \\
\hline
\hline
\end{tabular}
\begin{tablenotes} 
\item $a$ : Radial velocity of the RCB star, rounded to nearest 50 km s$^{-1}$. 
\item $b$ : Photospheric temperature of the RCB star. The uncertainty on the value is 250 K.
\item $c$ : Oxygen isotope ratios. The values are uncertain by a factor of two.
\end{tablenotes}
\end{minipage}
\end{table*}
\endgroup

==> table_temps.tex <==
\begingroup
\renewcommand{\tabcolsep}{2pt}
\begin{table*}
\begin{center}
\begin{minipage}{16cm}
\caption{Effective temperatures and isotope ratios of RCBs}
\label{tab:temps}
\begin{tabular}{ccc}
\hline
\hline
{RCB} & {T$_{\mathrm{eff}}$} & {O$^{16}$/O$^{18}$} \\ 
{} & {K} & {} & {}  \\
\hline
 &  &  \\
 &  &  \\
\hline
\hline
\end{tabular}
\begin{tablenotes} \item References: \end{tablenotes}
\end{minipage}
\end{center}
\end{table*}
\endgroup
